Relating Metric Distortion and Fairness of Social Choice Rules

One way of evaluating social choice (voting) rules is through a utilitarian distortion framework. In this model, we assume that agents submit full rankings over the alternatives, and these rankings are generated from underlying, but unknown, quantitative costs. The \emph{distortion} of a social choice rule is then the ratio of the total social cost of the chosen alternative to the optimal social cost of any alternative; since the true costs are unknown, we consider the worst-case distortion over all possible underlying costs. Analogously, we can consider the worst-case \emph{fairness ratio} of a social choice rule by comparing a useful notion of fairness (based on approximate majorization) for the chosen alternative to that of the optimal alternative. With an additional metric assumption -- that the costs equal the agent-alternative distances in some metric space -- it is known that the Copeland rule achieves both a distortion and fairness ratio of at most 5. For other rules, only bounds on the distortion are known, e.g., the popular Single Transferable Vote (STV) rule has distortion $O(\log m)$, where $m$ is the number of alternatives. We prove that the distinct notions of distortion and fairness ratio are in fact closely linked -- within an additive factor of 2 for any voting rule -- and thus STV also achieves an $O(\log m)$ fairness ratio. We further extend the notions of distortion and fairness ratio to social choice rules choosing a \emph{set} of alternatives. By relating the distortion of single-winner rules to multiple-winner rules, we establish that Recursive Copeland achieves a distortion of 5 and a fairness ratio of at most 7 for choosing a set of alternatives.

==> sets_graph.tex <==
\begin{center}
 \begin{tikzpicture}
	\tikzstyle{dot} = [draw, fill, circle, inner sep=1.5pt]
	\tikzstyle{set} = [draw, ellipse, inner sep=1.5pt]
	
	\node[matrix, name path=algborder] (alg) at (0.75,1) [set] {
		\node at (0,0) [dot] {}; 
        \node at (1.5,0) [dot] {};
        \node at (3,0) {$\cdots$};
        \node at (4.5,0) [dot] {}; \\
	};
	\node at (alg) [left=3.25cm] {$f(\sigma)$};
	\node[matrix, name path=optborder] (opt) at (5.25,1) [set] {
		\node at (0,0) [dot] {}; 
        \node at (1.5,0) {$\cdots$};
        \node at (3,0) [dot] {};
        \node at (4.5,0) [dot] {}; \\
	};
	\node at (opt) [right=3.25cm] {$\wopt$};
	
	\node (v) at (3,-1) [dot] {};
	\node at (v) [below] {$v$};
	
	\node (s1) at (3,2.65) [dot] {};
	\node (s2) at (3,3.5) [dot] {};
	\node (s3) at (3,4) [dot] {};
	\node at (3,3.15) {$\vdots$};
	\node at (3,4.5) {$S_k$};
	\draw (3,3.3) ellipse (0.5cm and 1cm);
	

	\path [name path=algs1] (s1) -- ($ (alg.west)!0.25!(alg) $);
    \draw [name intersections={of=algborder and algs1}]
                              (s1) -- (intersection-1);
	\path [name path=algs2] (s2) -- ($ (alg.west)!0.25!(alg) $);
    \draw [name intersections={of=algborder and algs2}]
                              (s2) -- (intersection-1);
	\path [name path=algs3] (s3) -- ($ (alg.west)!0.25!(alg) $);
    \draw [name intersections={of=algborder and algs3}]
                              (s3) -- (intersection-1)
                              node [midway,sloped,above] {$f_k$};
	\path [name path=algv] (v) -- ($ (alg.west)!0.25!(alg) $);
    \draw [name intersections={of=algborder and algv}]
                              (v) -- (intersection-1)
                              node [midway,sloped,below] {$\geq \frac{f_k-g_k}{k} - d(v,\wopt)$};
                              
    \path [name path=opts1] (s1) -- ($ (opt.east)!0.25!(opt) $);
    \draw [name intersections={of=optborder and opts1}]
                              (s1) -- (intersection-1);
	\path [name path=opts2] (s2) -- ($ (opt.east)!0.25!(opt) $);
    \draw [name intersections={of=optborder and opts2}]
                              (s2) -- (intersection-1);
	\path [name path=opts3] (s3) -- ($ (opt.east)!0.25!(opt) $);
    \draw [name intersections={of=optborder and opts3}]
                              (s3) -- (intersection-1)
                              node [midway,sloped,above] {$\leq g_k$};
	\path [name path=optv] (v) -- ($ (opt.east)!0.25!(opt) $);
    \draw [name intersections={of=optborder and optv}]
                              (v) -- (intersection-1)
                              node [midway,sloped,below] {$d(v,\wopt)$};

\end{tikzpicture}
\end{center}

